Improved linearly ordered colorings of hypergraphs via SDP rounding

We consider the problem of linearly ordered (LO) coloring of hypergraphs. A hypergraph has an LO coloring if there is a vertex coloring, using a set of ordered colors, so that (i) no edge is monochromatic, and (ii) each edge has a unique maximum color. It is an open question as to whether or not a 2-LO colorable 3-uniform hypergraph can be LO colored with 3 colors in polynomial time. Nakajima and \v{Z}ivn\'{y} recently gave a polynomial-time algorithm to color such hypergraphs with $\widetilde{O}(n^{1/3})$ colors and asked if SDP methods can be used directly to obtain improved bounds. Our main result is to show how to use SDP-based rounding methods to produce an LO coloring with $\widetilde{O}(n^{1/5})$ colors for such hypergraphs. We show how to reduce the problem to cases with highly structured SDP solutions, which we call balanced hypergraphs. Then, we discuss how to apply classic SDP-rounding tools to obtain improved bounds.

==> simple-coloring.tex <==
\section{Coloring of 2-LO Colorable 3-Uniform Hypergraphs}\label{app:simple2color}

In this section, we show how to color a 2-LO colorable 3-uniform
hypergraph with 2 colors.  For simplicity, we define {\em balanced}
vertices to be those with $\gamma_a = -1/3$.  It is straightforward to
extend to the case of $\eps$-balanced for small but (strictly)
positive $\eps$.

\begin{algorithm}[H]
\caption{2-Coloring Algorithm}
\label{alg:two-color}
Input: A solution to \prettyref{sdp:lo_coloring}.\\
Two-Sided Combinatorial Rounding
\begin{enumerate}
	\item Set
		$S_l \assign \set{a\in V \given \gamma_a<-\frac{1}{3}}$,
		$S_r \assign \set{a\in V \given \gamma_a>-\frac{1}{3}}$, and
		$S_b \assign \set{a \in V \given \gamma_a = -\frac{1}{3}}$.
	\item Color $S_l$ using color 1 and $S_r$ using color 2.
\end{enumerate}
Two-Sided Hyperplane Rounding
\begin{enumerate}[resume]
	\item Choose a uniformly random unit vector $r$ over the sphere.
	\item Set $H_r \assign \set{a\in S_b \given \inprod{r, \vectu{a}}\geq 0}$ and $H_l \assign \set{a\in S_b \given \inprod{r, \vectu{a}}< 0}$.
	\item Color $H_l$ using 1 and $H_r$ using 2.
\end{enumerate}

\end{algorithm}

\begin{lemma}
	\label{lem:two-color-comb}
Let $S_l$, $S_r$ be as defined in \prettyref{alg:two-color}.
Then, for any edge $e\in E$, we have $S_l\cap e\ne \emptyset$ if and only if $S_r\cap e\ne \emptyset$.
\end{lemma}

\begin{proof}
	Fix an edge $\set{a, b, c}=e\in E$.
	\prettyref{obs:vect-prop} states that $\gamma_a+\gamma_b+\gamma_c=-1$
	Suppose that $e\cap S_l\ne \emptyset$ and $e\subseteq S_l\cup S_b$.
	Then, we get $\gamma_a+\gamma_b+\gamma_c<-1$, a contradiction.
	Hence, $e\cap S_l\ne \emptyset$ implies $e\cap S_r\ne \emptyset$
	The proof of the converse is similar.
\end{proof}


\begin{lemma}
	\label{lem:two-color-half}
	Let $r$ be unit vector distributed uniformly over the sphere and let $H_l$, and $H_r$ be defined as in \prettyref{alg:two-color}.
	Then,  for any edge $e\in E$, we have $\card{H_l\cap e}\leq 2$ and $\card{H_r\cap e}\leq 2$ (with probability 1).
\end{lemma}
\begin{proof}
	We can assume that $H_r=\set{a\in S_b | \inprod{r, \vectu{a}}> 0}$,
	as this is true with probability 1.
	Fix any $e\in E$. 
	Assume that $\set{a, b, c}=e\subseteq S_b$; otherwise, we are done.
	Using \prettyref{lem:u_bound} with $\eps=0$
	we get $\norm{\vectu{a}+\vectu{b}+\vectu{c}}^2 =0$,
	which implies $\vectu{a}+\vectu{b}+\vectu{c}=0$.
	Therefore, we have $\inprod{r, \vectu{a}}+\inprod{r, \vectu{b}} + \inprod{r, \vectu{c}}=0$.
	But, if $e\subseteq H_l$, then we have $\inprod{r, \vectu{a}}+\inprod{r, \vectu{b}} + \inprod{r, \vectu{c}}<0$, a contradiction.
	Similarly, if $e\subseteq H_r$, then we have a contradiction in form of $\inprod{r, \vectu{a}}+\inprod{r, \vectu{b}} + \inprod{r, \vectu{c}}>0$.
\end{proof}

\begin{theorem}
	There is a polynomial-time algorithm that, if given a 2-LO colorable 3-uniform hypergraph $H$ with $n$ vertices, finds an 2-coloring of $H$. 
\end{theorem}
\begin{proof}
	Solve \prettyref{sdp:lo_coloring} and use \prettyref{alg:two-color}.
	Consider any edge $e = \set{a, b, c}$.
	If $e$ is not completely contained in $S_b$,
	then by \autoref{lem:two-color-comb} we at least
	one vertex each from $S_l$ and $S_r$; hence, $e$ is non-monochromatic.
	Otherwise, $e$ is non-monochromatic by \autoref{lem:two-color-half}.
\end{proof}

